Safety Aware Reinforcement Learning (SARL)

As reinforcement learning agents become increasingly integrated into complex, real-world environments, designing for safety becomes a critical consideration. We specifically focus on researching scenarios where agents can cause undesired side effects while executing a policy on a primary task. Since one can define multiple tasks for a given environment dynamics, there are two important challenges. First, we need to abstract the concept of safety that applies broadly to that environment independent of the specific task being executed. Second, we need a mechanism for the abstracted notion of safety to modulate the actions of agents executing different policies to minimize their side-effects. In this work, we propose Safety Aware Reinforcement Learning (SARL) - a framework where a virtual safe agent modulates the actions of a main reward-based agent to minimize side effects. The safe agent learns a task-independent notion of safety for a given environment. The main agent is then trained with a regularization loss given by the distance between the native action probabilities of the two agents. Since the safe agent effectively abstracts a task-independent notion of safety via its action probabilities, it can be ported to modulate multiple policies solving different tasks within the given environment without further training. We contrast this with solutions that rely on task-specific regularization metrics and test our framework on the SafeLife Suite, based on Conway's Game of Life, comprising a number of complex tasks in dynamic environments. We show that our solution is able to match the performance of solutions that rely on task-specific side-effect penalties on both the primary and safety objectives while additionally providing the benefit of generalizability and portability.

==> Neurips-2020-version/broader-impacts.tex <==
\section{Broader Impacts}
Broader Impacts section per Neurips requirement

==> Neurips-2020-version/discussion.tex <==
\section{Discussion} \label{discussion}
% \begin{itemize}
%     \item \textcolor{blue} {Regularization ideas: Talk about how proper distance metrics express something meaningful}
%     \item \textcolor{blue} {Future work on different safety metrics discussing limitations of the current metric}
%     \item \textcolor{blue} {Extending to continuous environments (Safetygym) and continuous algorithms}
%     \item \textcolor{blue} {integrating motion planning type approaches such as reachability}
%     \item \textcolor{blue} {other Wasserstein formulation than Sinkhorn (Sinkhorn makes most sense due to speed and differentiability}
% \end{itemize}

We believe that this work shows the promise of using a co-training framework to train RL agents in environments where side effects are important. As mentioned in \ref{introduction}, side effects are often difficult to define, especially when interwoven with the primary task, and therefore measuring and interpreting side effects is an continuing research work. Given the hope and expectation that the ability to measure side effects will continue to evolve in the future, we designed our co-training framework to be flexible to different side effect metrics that can be integrated as research in the field progresses. \par

We also believe that the idea of using proper distance metrics to perform co-training of RL agents has a variety of future research directions. One such avenue is the development of new distance metrics, including variations of the Wasserstein Distance other than the Sinkhorn Distance used in our study, as well as distance metrics can exploit various channels of information to help training like the Jensen-Shannon Distance in our experiments. The ideal distance metric would capture both the information richness from the different channels and encode a notion of side effect, or another safety objective, that can be transferred to the primary agent to influence its behavior. We believe that the field of distance metrics between various kinds of distributions continuous to provide many important and impactful research questions that can be transferred to a large array of fields, including reinforcement learning as we have shown in this work. \par

Lastly, the Q-learning co-training framework we proposed focused exclusively discrete action spaces which do not capture the full extent of RL algorithms and environments. As such, a natural extension of this work is to develop a framework for continuous action spaces that builds on the ideas presented in this work. Many continuous space algorithms have a variety of agents, such as actors and critics, working together to achieve a common objective. We believe that integrating the idea of virtual agent co-training with proper distance metrics can upon up new algorithmic designs to tackle side effect scenarios as well as other safety critical applications in reinforcement learning. Moreover, since a proper distance is agnostic to where the distribution came from, we believe this opens the possibility for integrating algorithms and techniques from motion planning and other classical control models with model free reinforcement learning algorithms. We believe that this could be particularly valuable in safety critical applications given the long history of safety research in classical control algorithms.

\textcolor{red}{Potential discussion on distance metric learning}

==> Neurips-2020-version/intro.tex <==
% \textbf{General Flow - Topic Sentences}
% \begin{itemize}
%     \item Introduction
%     \begin{itemize}
%         \item Introduction: RL and Safety
%         \item RL and Regularization for Robustness (Abdullah work and Pacciona)
%         \item Safelife as discrete action space environment for side effects
%         \item Side-effect inspired regularization
%         \item Discussion on distance metrics
%         \item Summary of contributions
%     \end{itemize}
%     \item SafeLife
%     \begin{itemize}
%         \item Safelife as procedurally generating environments for side effects
%         \item still environments and the current side-effect metric
%         \item dynamic environments and the shortfall of the side effect metric (and lack of a good one in general)
%     \end{itemize}
%     \item Method
%     \begin{itemize}
%         \item Co-training diagram with DDQN relationships
%         \item Distance metrics (JS and WD) and their foundations (mutual information and earth mover) and basis for using them to measure distance and bias the agent
%         \item overall algorithm flow
%     \end{itemize}
%     \item Result
%     \begin{itemize}
%         \item Still environments with different distances - safety tradeoff for prune; append funky - harder task, harder to be safet (especially when standard is low)
%         \item Dynamic environments showing better sample efficiency (maybe leave off side effects as the meaning is unclear)
%     \end{itemize}
%     \item Discussion
%     \begin{itemize}
%         \item the effects of the different distances and the flexibility of the framework to handle different setups
%         \item Future Work: port to continuous environments and algorithms like SafetyGym
%         \item Safety metric to better capture dynamic environments and apply them with current framework
%         \item integrating of a more planning based approach based on control literature and building that bridge
%         \item other variations of Wasserstein like in \citep{Abdullah2019}
%     \end{itemize}
    
% \end{itemize}

\section{Introduction} \label{introduction}
% \begin{itemize}
%     \item \textcolor{blue} {General Literature Review of Safety in RL with the 9 problems from Amodei}
%     \item \textcolor{blue} {Limitations of current environments and introduction to Safelife - describe the different tasks and settings in Safelife}
%     \item \textcolor{blue} {Summarize main contributions}
%     \item \textcolor{red}{include discussion on "soft" state of the side effect metric and how that differs from traditional motion planning where the model and estimation of reach-ability are much more clearly defined}
% \end{itemize}

Reinforcement learning (RL) algorithms have seen great research advances in recent years, both in theory and in their applications to concrete engineering problems. The application of RL algorithms extends to computer games (\citep{mnih2013playing}; \citep{silver2017mastering}), to robotics (\citep{gu2017deep}) and recently real-world engineering problems, such as microgrid optimization \citep{liu2018distributed} and hardware design \citep{mirhoseini2020chip}. As RL agents become more and more prevalent in complex real-world applications, the notion of safety becomes more and more important. Given the increasing importance of safety in RL, safety related research in RL has also seen a significant surge in recent years.



% Early work by \cite{amodei2016safetyproblems} classified safety problems in RL into 9 distinct categories, while \citep{leike2017safetygrids} developed elementary gridworld environments to investigate how common RL algorithms perform in relatively simple scenarios where safety and task performance are important. The questions identified by \citep{amodei2016safetyproblems} included: 

%  \begin{itemize}
%     \item \textbf{Avoiding Side Effects} (Amodei et al., 2016): How can we get agents to minimize effects unrelated to their main objectives, especially those that are irreversible or difficult to re- verse?
%     \item \textbf{Safe Interruptibility} (Orseau and Armstrong, 2016): We want to be able to interrupt an agent and override its actions at any time. How can we design agents that neither seek nor avoid interruptions?
%     \item \textbf{Absent Supervisor} (Armstrong, 2017): How we can make sure an agent does not behave differently depending on the presence or absence of a supervisor?
%     \item \textbf{Reward Gaming} (Clark and Amodei, 2016): How can we build agents that do not try to introduce or exploit errors in the reward function in order to get more reward?
%     \item \textbf{ Self-Modification} How can we design agents that behave well in environments that allow self-modification
%     \item \textbf{Distributional Shift} (Qui{\~n}onero Candela et al., 2009): How do we ensure that an agent behaves robustly when its test environment differs from the training environment?
%     \item \textbf{Robustness to Adversaries} (Auer et al., 2002; Szegedy et al., 2013): How does an agent detect and adapt to friendly and adversarial intentions present in the environment?
%     \item \textbf{Safe Exploration} (Pecka and Svoboda, 2014): How can we build agents that respect safety constraints not only during normal operation, but also during the initial learning period?
% \end{itemize}

\subsection{Side Effects in Reinforcement Learning Environments}
% \textcolor{blue}{Make sure that this is not safe exploration - you end up with a safe policy and are OK during exploration}
Our work focuses specifically on the safety problem of side effects, specified as one of the categories by \citep{amodei2016safetyproblems}, where an agent's actions to perform a task in its environment may cause undesired, and sometimes irreversible, changes in the environment. The problem of side effects in a given environment is still fairly opaque, as general measures of side effects are often engineered to the given task and environment and often do not generalize beyond a limited setting. The side effect scenario is also distinctly different from safe exploration and the traditional motion planning task, where one can formulate the goal of the algorithm in terms of reaching a goal state and avoiding obstacles. Unlike obstacles, side effects are more broadly defined, and their relationship with the primary task can also more convoluted than in traditional motion planning depending on the nature of the task and the environment. As such, many of the traditional safety approaches do not scale well to the side effect scenarios we consider. For one, when learning a task in an unknown environment with complex dynamics, it is challenging to formulate an appropriate model to jointly encapsulate the task and side effect problem. This will in turn make it difficult to use approaches from motion planning methods, as well reward hacking type setups where the side effects is included in the reward function of the environment. Previous work on formulating a more precise definition of side effects includes work by \citep{turner2019aup} on conservative utility preservation and by \citep{krakovna2018penalizing} on relative reachability have investigated more abstract notions of measuring side effects based on a deeper analysis of changes, reversible and irreversible, in the state space itself. While those works have made great progress on advancing towards a greater understanding of side effects, their studies have generally been limited to gridworld environments where the RL problem can often be solved in a tabular way and value function estimations are often not prohibitively demanding. Given the limitations of gridworld environments, our work focuses on expanding the concept of side effects to more complex environments, generated by the SafeLife suite, with more intricate function estimations embedded in a flexible architecture. The training framework we developed is a novel architecture that learns from both reward and side effect information in a co-training fashion and is therefore flexible to various environment, task and side effect definitions. This co-learning architecture is metaphorically similar to a integrating a safety conscience into the reward agent that influences the actions of the agent in the environment, leading to the name Conscience Aware Deep Q-Networks (CA-DQN).
Based upon SC-DQN, we propose the following contributions, which to the best of our knowledge are novel addition to the growing field of research in RL safety:
% \textcolor{blue}{Train safe agents in more general way without limiting other work on side effects - Architectural argument for making sure that this flexible and given choice of metric, environment, policy, we can systematically train.} 

\begin{itemize}
    \item CA-DQN: A flexible RL co-training framework for discrete action spaces based on DDQN that can be applied to complex discrete action environments, which is agnostic to the side effect metric used in the environment.
    \item A regularization method of the DDQN loss metric for safety and reward co-training based on the notion of distance between probability distribution, specifically the Jensen-Shannon Distance and Sinkhorn Distance, a variant of the Wasserstein Distance, building on multipolicy regularization work by \citep{Pacchiano2019} and \citep{Abdullah2019}. The notion of using a distance expresses the difference in the distribution of safe and purely reward based, which allow the agent to take actions that are more aligned with the safe distribution of actions while still optimizing the primary reward. The formulation of the distances lead to two primary emerging behaviors:
    \begin{itemize}
        \item When the safety metric is accurately described by the environmental information channel, agents regularized with the soft metric given by the Jensen-Shannon Distance matches or improves upon primary task while usually yielding minimal improvements in the safety metric. Agents regularized with the hard metric Sinkhorn Distance, on the other hand, show that safer behavior can be achieved but often at a performance cost.
        \item In environments where the safety metric is incomplete, such as dynamic environments with natural variation, agents regularized with the Jensen-Shannon Distance still matches or improves upon the primary task performance due to mutual information exchange between the different information channels. Agents regularized with the hard Sinkhorn Distance, however, tend to highly favor safe actions at the excessive expense of primary task performance.
    \end{itemize}

\end{itemize}
We provide a description of the SafeLife suite in Section \ref{safelife-env}, a detailed description of our RL method in Section \ref{method}, our experiments and results for various environments in Section \ref{results} as well as a discussion in Section \ref{discussion}.

==> Neurips-2020-version/method.tex <==


\section{Method} \label{method}
% \begin{itemize}
%     \item \textcolor{blue} {Brief descriptions of DDQN}
%     \item \textcolor{blue} {Diagram with Safe DDQN and description}
%     \item \textcolor{blue} {Distance Metric Section with discussion on JS and Sinkhorn}
%     \item \textcolor{blue} {Regular and Repulsive Formulations for regularization}
%     \item \textcolor{blue} {final pseudocode - can use color coding similar to image augmentation in RL paper}
% \end{itemize}

\subsection{Co-Training for Regularized Safe RL Agent}
Our method is an extension of DDQN \citep{ddqn-hasselt} that consists of a reward agent (the actor), $A(\theta)$, and a virtual safety, $Z(\psi)$,  agent shown in Figure \ref{fig:co-training}. The safety agent is virtual, because it does take any actions but issues recommendations to the actor through regularization of the actor's loss function.
\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth, height= 0.66\linewidth]{images/Safe Co-Training.png}
    \caption{A co-training framework for safety aware RL training. The reward agent (actor),  $A(\theta)$, determines the action taken in the environment and the resulting trajectories. The reward and safety metric are stored in separate replay buffers for the same agent trajectories. The safety agent, $Z(\psi)$, samples from its replay buffer to train on the safety metric in regular DDQN fashion. The reward agent samples from its replay buffer, computes the DDQN which is then regularized by the safety agent through a distance metric between the normalized outputs of Q-functions of the reward and safety agent.}
    \label{fig:co-training}
\end{figure}
In this framework, the virtual safe agent follows the trajectories of the actor and learns to predict the expected return of the safety metric based on the trajectory of the reward agent. The virtual safe agent is optimized using the DDQN algorithm described in \citep{ddqn-hasselt}: $Z(\psi)$ samples a batch of states $\mathcal{S}$ from its replay buffer and computes 
\begin{align*}
    \mathcal{L}(\psi) &= \lVert Q_t^{Z}(\mathcal{S},\mathcal{A}) - Y_t^{DDQN} \rVert \tag{1} \label{eq:safe_lossl} \\
    &= \lVert Q_t^{Z}(\mathcal{S},\mathcal{A}) - (\zeta_{t+1} + \gamma Q(\mathcal{S}_{t+1},\underset{a}{\argmax} Q(\mathcal{S}_{t+1},a, \psi_t);\psi_t^{\prime}) \rVert  
\end{align*}
where $\mathcal{\zeta}$ is the safety metric given by the environment. The actor, $A(\theta)$, has the following regularized loss function
\begin{align*}
    \mathcal{L_A}(\theta) &= \beta*\mathcal{L}^{DDQN}_{\theta} + (1 - \beta)*\infdiv{\rho(\theta)}{\omega(\psi)}    \tag{2} \label{eq:actor_loss} \\
\end{align*}
where $\beta$ is a regularization hyperparameter,$\rho(\theta)$ represents the probability of taking an action according to the Q-Values of the reward and $\omega(\psi$ represent the probability distribution of taking according to the Q-Values of the safe virtual agent. As shown in Equation \ref{eq:actor_loss}, the actor loss $\mathcal{L}(\theta)$ is regularized by the distance between the actions suggested by the reward-based actor and the safe virtual agent. 
The regularization is positive when the virtual agent wants to bias the actor towards its own behavior and negative when the virtual agent wants to bias the actor away from its own behavior. 
\begin{align*}
    \mathcal{L_A}(\theta) &= \beta*\mathcal{L}^{DDQN}_{\theta} - (1 - \beta)*\infdiv{\rho(\theta)}{\omega(\psi)}    \tag{2} \label{eq:actor_loss-repulsive} \\
\end{align*}
This repulsive formulation can be used by teaching the virtual agent unsafe behavior and then discourage the actor from those actions. In our implementation of the repulsive formulation, the replay buffer of the virtual agent $\mathcal{R}^Z$ stores the opposite sign of the side effect metric, thereby wanting to maximize side effects. We apply this repulsive formulation in the dynamic environments.

This distance metric needs to be differentiable to enable learning via backpropagation, and in the following section we discuss two choices we applied in our experiments: the Jensen-Shannon Divergence, a variation of the Kullback-Leibner (KL) Divergence, and the Sinkhorn Distance, a variation of the Wasserstein Distance.


\subsection{Distance Metrics for Regularization Loss}
\textcolor{blue}{Used distance metrics because they have certain properties, including symmetry, positive values and satisfy triangle inequality. This makes a more robust setup for information transfer.}
\subsubsection{Jensen-Shannon Distance}
The distance metric, $\infdiv{\rho(\theta)}{\omega(\psi)}$ provides the information exchange between the virtual safe agent $Z(\psi)$  and the actor $A(\theta)$. of taking a safe is  which is why it is important to apply a distance metric that expresses the goal of the regularization. In our case, we intend to measure the difference in the probabilities of taking a purely reward motivated action compared to taking a purely safety motivated action. We express that difference as an additional cost in the loss function of the actor via the regularization term. One method of measuring the difference in probability distributions is the KL Divergence, $D_{KL}(p \| q) = \int_x p(x) \log \frac{p(x)}{q(x)} dx$, where $p$ and $q$ are probability distributions. The KL divergence, however, is not a true distance metric as is it not symmetric given that $D_{KL}(p \| q) \neq D_{KL}(q \| p)$ and it does not satisfy the triangle inequality. As such, the KL divergence does not meet the requirements for measuring the distance between the distance between the distributions of taking a safe action and taking a purely reward motivated action. We therefore choose to use the Jensen-Shannon distance $D_{JS}(p \| q) = \frac{1}{2} D_{KL}(p \| q)+ \frac{1}{2} D_{KL}(q \| p )$, which is true distance metric based on the KL divergence as one of our distance metrics. In addition to satisfying the requirement of being a true distance, $D_{JS}$ is also a good fit becomes it measures the mutual information between the between the two distributions $p$ and $q$, which in our case translates to the mutual information between $\rho(\theta)$ and $\omega(\psi)$.
\subsubsection{Sinkhorn Distance}
The Sinkhorn distance is a surrogate of the Wasserstein distance which takes into account the metric space when measuring the distance between two probability distributions. The Wasserstein distance, defined as $W_p(P, Q) = 
(\inf_{J \in \mathcal{J}(P,Q)} \int \lVert x-y \rVert^p \mathrm{d}J(x,y))^{\frac{1}{p}}$, is commonly known as the earth mover as it measures how much work it would take to move one probability distribution $p$ to the $q$ assuming they were masses of earth. When the calculation of the Wasserstein is reformulated as an optimal transport problem, we arrive at the Sinkhorn distance \citep{Cuturi2013} $d_M \coloneqq \min_{P \in U(r,c)} \langle P,M \rangle$ which can be solved iteratively using the Sinkhorn algorithm. AS described in detail in \citep{Cuturi2013}, the Sinkhorn distance meets the desired metric properties and computes the resulting distances via entropy regularization by imposing on entropy constraint on the probability distributions. Moreover, the Sinkhorn algorithm includes entirely differentiable operations, making it suitable for our formulation. Our co-training framework includes an inner loop that computes the Sinkhorn distance $d_{M}(\rho(\theta) \| \omega(\psi))$ using the Pytorch framework. Whereas the Jensen-Shannon distance measures mutual information and provides a soft penalty for large divergence between $\rho(\theta)$ and $\omega(\psi)$, the Sinkhorn distance provides a hard penalty that aims to bring the distribution of $\rho(\theta)$ closer to $\omega(\psi)$.

\subsection{Safety Regularized Deep Q-Learning}
The paragraphs above in \ref{method} describe the pieces needed to put together the overall algorithm. Our current algorithm applies $\epsilon$-greedy exploration to pick the actions, but the algorithm is amendable to other exploration policies. \textcolor{red}{Discussion on the Softmax temperature parameter}

\vspace{\baselineskip}
\begin{algorithm}[]
\caption{CA-DQN}
\label{alg:co-train-algo} 
\begin{algorithmic}[1]
% \State \textcolor{red}{Add colors to have the steps for different agents}
\State Initialize an actor \textcolor{dark-blue}{$A(s|\theta)$} and virtual agent \textcolor{dark-green}{$Z(s|\psi)$}
\State Initialize target networks \textcolor{dark-blue}{$A^{\prime}$} and \textcolor{dark-green}{$Z^{\prime}$} with weights \textcolor{dark-blue}{$\theta^{A^{\prime}} \leftarrow \theta^A$}, \textcolor{dark-green}{$\psi^{Z^{\prime}} \leftarrow \psi^Z$}
\State Initialize a replay buffer \textcolor{dark-blue}{$\mathcal{R}^A$} storing rewards for the actor and \textcolor{dark-green}{$\mathcal{R}^Z$} storing side effects for the safe virtual agent
\State Initialize exploration policy, e.g. $\epsilon$-greedy
\State Set hyperparameters, including target update frequency for \textcolor{dark-blue}{$A(s|\theta)$} and \textcolor{dark-green}{$Z(s|\psi)$}

% \For{Episodes = 1, $N$}

    % \While{$\mathcal{R} < \mathcal{R}^{initial}$}
    %     \State Perform exploration in the environment according to exploration policy
    %     \State Store reward transitions $(s_i, a_i, r_i, s_{i+1})$ in $\mathcal{R}^A$ 
    %     \State Store side effect $(s_i, a_i, \zeta_i, s_{i+1})$ in $\mathcal{R}^Z$
    % \EndWhile
    
    % \State Receive initial observation state $s_0$
    
    \For{each environment episode}

        \State Select action \textcolor{dark-blue}{$a_t = A(\theta)$} according to exploration policy
        \State Execute action $a_t$ and observe reward \textcolor{dark-blue}{$r_t$}, side effect \textcolor{dark-green}{$\zeta_t$} and new state $s_{t+1}$
        \State Store reward transitions \textcolor{dark-blue}{$(s_i, a_i, r_i, s_{i+1})$} in \textcolor{dark-blue}{$\mathcal{R}^A$} 
        \State Store side effect \textcolor{dark-green}{$(s_i, a_i, \zeta_i, s_{i+1})$} in \textcolor{dark-green}{$\mathcal{R}^Z$}
        % \State \textbf{\emph{Virtual Agent}}
        \For{each virtual agent update}
        \State Sample a random minibatch of $N$ transitions \textcolor{dark-green}{$(s_i, a_i, \zeta_i, s_{i+1})$} from \textcolor{dark-green}{$\mathcal{R}^Z$ }
        \State Set \textcolor{dark-green}{$y_i^\zeta = (\zeta_{i} + \gamma Q^{\prime}(s_{t+1},A^{\prime}(s_{t+1}|\theta^{A^{\prime}})$}
        \State Update virtual agent by minimizing loss \textcolor{dark-green}{$\mathcal{L}(\psi) = \frac{1}{N} \sum_i (y_i^{\zeta} -  Q^{Z}(s_i,\psi) )^2$}
        \EndFor
        % \State \textbf{\emph{Actor}}
        \For{each actor update}
        \State Sample a random minibatch of $N$ transitions \textcolor{dark-blue}{$(s_i, a_i, r_i, s_{i+1})$} from \textcolor{dark-blue}{$\mathcal{R}^A$ }
        \State  Set \textcolor{dark-blue}{$y_i^r = (r_{i} + \gamma Q^{\prime}(s_{t+1},A^{\prime}(s_{t+1}|\theta^{A^{\prime}})$}
        \State  Compute \textcolor{dark-blue}{$\mathcal{L}_{\theta} = \frac{1}{N} \sum_i (y_i^{r} -  Q^{A}(s_i,\theta) )^2$}
        \vspace{\baselineskip}
        \State \textbf{\emph{Distance Computation}}
        \State Compute  \textcolor{dark-green}{$Q^Z(s_i,\psi)$} and  \textcolor{dark-green}{$Q^Z(s_{i+1},\psi)$}
        
        \State Compute actor action probabilities  \textcolor{dark-blue}{$\rho_t^A = \frac{e^{Q^A(s_t,\theta)}}{\sum e^{Q^A(s_t,\theta)}}$,  $\rho_{t+1}^A = \frac{e^{Q^A(s_{t+1},\theta)}}{\sum e^{Q^A(s_{t+1},\theta)}}$}
        
        \State Compute virtual agent action probabilities  \textcolor{dark-green}{$\omega_t^Z = \frac{e^{Q^Z(s_t,\psi)}}{\sum e^{Q^Z(s_t,\psi)}}$,  $\omega_{t+1}^Z = \frac{e^{Q^Z(s_{t+1},\theta)}}{\sum e^{Q^Z(s_{t+1},\psi)}}$}
        \vspace{\baselineskip}
        
        \State Compute $\textcolor{dark-red}{\mathcal{L}_{Div}} = \textcolor{dark-red}{Div}( \textcolor{dark-blue}{\rho_t^A }\|  \textcolor{dark-green}{\omega_t^Z)} + \gamma*\textcolor{dark-red}{Div}( \textcolor{dark-blue}{\rho_{t+1}^A} \|  \textcolor{dark-green}{\omega_{t+1}^Z)}$
        \vspace{\baselineskip}
        \State Update actor policy using  $\textcolor{dark-blue}{\mathcal{L}_A(\theta)} = \beta\textcolor{dark-blue}{\mathcal{L}_{\theta}} + (1-\beta)\textcolor{dark-red}{\mathcal{L}_{Div}}$
        \EndFor
        \State Update target networks $ \textcolor{dark-blue}{\theta^{A^{\prime}} \leftarrow \theta^A},  \textcolor{dark-green}{\psi^{Z^{\prime}} \leftarrow \psi^Z}$
        
        
    \EndFor
% \State \textcolor{red}{Add colors to have the steps for different agents}
% \EndFor
\end{algorithmic}
\end{algorithm}

The co-training algorithm is agnostic to the side effect metric used in the environment, leading itself to a plug-and-play approach where the virtual agent can advise on a variety of different metrics without major modification to the overall structure of the method.

==> Neurips-2020-version/results.tex <==
\section{Results} \label{results}
% \begin{itemize}
%     \item \textcolor{blue} {Navigate}
%     \item \textcolor{blue} {Static Environments - Prune Hard and Append}
%     \item \textcolor{blue} {Dynamic Environments}
% \end{itemize}

\subsection{Navigation Task}
The navigation task is the simplest of the SafeLife task, which includes the agent navigating from a starting point to the level exit. For this task, as with all tasks shown in the results, the co-training agent are compared to a DDQN baseline trained without the SafeLife impact penalty and with the SafeLife impact penalty. 

\begin{figure}[ht]%\hspace*{\fill}

\subfigure[Navigation Episode Length]{
\includegraphics[width=0.5\columnwidth]{Doc_images/Navigate_episodes_length.png}}\hspace*{\fill}
\subfigure[Navigate Side Effects]{
\includegraphics[width=0.5\columnwidth]{Doc_images/Navigate_episodes_effects.png}}\hspace*{\fill}
\caption{(a) Episode Length for the Navigation Task with Various Algorithms (b) Side Effect metric based on the starting state for various algorithms}
\label{fig:nav-fig}
\vspace{1em}
\end{figure}
 As shown in Figure \ref{fig:nav-fig} using a penalty based formulation directly on the reward function fails to learn the main task, while the co-training framework matches the performances of the original DDQN baseline on the primary task. The Sinkhorn regularized actor actually matches the performance of the DDQN baseline while performing the task in a safer way as seen in the lower count of the side effect metric.
 
 \subsection{Prune Task}
 For the prune task, the agent needs to remove red automata from the board and then reach the level exit. This task is more involved than simple navigation and has a significantly larger state space. The episode length serves a proxy for task performance, as the agent reaches the level exit faster after completing the required task.
 
 \begin{figure}[ht]%\hspace*{\fill}

\subfigure[Prune Task Episode Length]{
\includegraphics[width=0.33\columnwidth]{Doc_images/Prune_Hard_episodes_length.png}}\hspace*{\fill}
\subfigure[Prune Task Side Effects]{
\includegraphics[width=0.33\columnwidth]{Doc_images/Prune_Hard_episodes_effects.png}}\hspace*{\fill}
\subfigure[Prune Task Performance]{
\includegraphics[width=0.33\columnwidth]{Doc_images/Prune_Hard_episodes_effects.png}}\hspace*{\fill}
\caption{(a) Episode Length for the Prune Task with Various Algorithms (b) Side Effect metric based on the starting state for various algorithms (c) Performance measured in the fraction of possible reward for various algorithms}
\label{fig:prune-fig}
\vspace{1em}
\end{figure}

AS shown in Figure \ref{fig:prune-fig}, the penalty formulation fails to learn the task while the agent regularized Jensen-Shannon Distance matches the baseline DDQN agent in both task performance and side effect metrics. The agent regularized by the Sinkhorn Distance shows a noticeable improvement in the side effect metric, which comes at a performance cost as the agent takes longer to complete the episode.

\subsection{Append Task}
The append task is the hardest of the SafeLife suite task; it involves filling in pattern on the board where the automata placed by the agent follow the same rules as the other automata on the board. This task can get especially difficult depending not only on the layout of the desired pattern, but also the presence of other automata on the board that can greatly complicate the interactions between the automata. This higher degree of complexity not only weighs on the task performance, but also on the ability to contain side effects

 \begin{figure}[ht]%\hspace*{\fill}

\subfigure[Append Task Episode Length]{
\includegraphics[width=0.33\columnwidth]{Doc_images/Append_still_episodes_length.png}}\hspace*{\fill}
\subfigure[Append Task Side Effects]{
\includegraphics[width=0.33\columnwidth]{Doc_images/Append_still_episodes_effects.png}}\hspace*{\fill}
\subfigure[Append Task Performance]{
\includegraphics[width=0.33\columnwidth]{Doc_images/Append_still_episodes_performance.png}}\hspace*{\fill}
\caption{(a) Episode Length for the Append Task with Various Algorithms (b) Side Effect metric based on the starting state for various algorithms (c) Performance measured in the fraction of possible reward for various algorithms}
\label{fig:append-fig}
\vspace{1em}
\end{figure}

As seen in \ref{fig:append-fig}, the penalty formulation does improve the side effect metric at the cost of task performance. The agent regularized by the Sinkhorn Distance initially improves the side effect score at the expense of task performance, but then converges towards the side effect score the main agent. \textcolor{red}{This could indicate that the Sinkhorn agent initally takes a safer path, but the side effects of the environments are difficult to control beyond the metric achieved by the baseline.} In this case, the Jensen-Shannon agent actually learns faster than the baseline while maintaining side effect performance. This indicates that the Jensen-Shannon agent is exploiting the mutual information given by the virtual agent that actually helps on task performance for a more complex overall setting.

\subsection{Dynamic Environments}
The phenomenon that the Jensen-Shannon regularized agents improve sample efficiency for more complex setups is also seen in the dynamic environments, where there is natural variation in the SafeLife board caused by the environment itself. This makes it difficult to evaluate side effects based on the default SafeLife metric that measures the change of the board compared to the initial state of the episode, as the natural variation changes the state of the board with or without agent interaction in the environment. This added complexity further makes it difficult for the baseline agents to learn the task effectively and using safety penalties virtually destroys the ability to improve task performance. 

 \begin{figure}[ht]%\hspace*{\fill}

\subfigure[Prune Dynamic Episode Length]{
\includegraphics[width=0.4\columnwidth]{Doc_images/Prune_dynamic_episodes_length.png}}\hspace*{\fill}
\subfigure[Append Dynamic Episode Length]{
\includegraphics[width=0.4\columnwidth]{Doc_images/Append_dynamic_episodes_length.png}}\hspace*{\fill}
\caption{(a) Episode Length for the Prune Task in Dynamic Environment (b) Episode Length for the Append Task in Dynamic Environment}
\label{fig:append-fig}
\vspace{1em}
\end{figure}


Moreover, even using the harder Sinkhorn Distance makes learning the primary task very challenging. The Jensen-Shannon agents, however, learn the tasks with greater sample efficiency, which reinforces the idea that the more complex the setting becomes (whether through a more complex environment or a more complex task), the more important mutual information becomes for solving the primary task more efficiently. This indicates that using multiple channels of information is beneficial for improving primary task performance, including if the other channel is a flawed side effect metric that provides limited information. 
\textcolor{blue}{Add points and discussion on the video that can add to the arguments above}

==> Neurips-2020-version/safelife.tex <==
\newcommand{\inlinesprite}[1]{
  \begingroup\normalfont\hspace{-0.5em}
  \raisebox{-.1\height}{\includegraphics[height=0.65em, clip, trim={#1}]{images/sprites-gray.pdf}}
  \hspace{-0.22em}\endgroup
}
\DeclareRobustCommand {\agentsprite}    {\inlinesprite{2cm 4cm 2cm 0cm}}
\DeclareRobustCommand {\lifesprite}     {\inlinesprite{0cm 3cm 4cm 1cm}}
\DeclareRobustCommand {\hardlifesprite} {\inlinesprite{1cm 3cm 3cm 1cm}}
\DeclareRobustCommand {\weedsprite}     {\inlinesprite{2cm 3cm 2cm 1cm}}
\DeclareRobustCommand {\plantsprite}    {\inlinesprite{3cm 3cm 1cm 1cm}}
\DeclareRobustCommand {\treesprite}     {\inlinesprite{3cm 1cm 1cm 3cm}}
\DeclareRobustCommand {\icesprite}      {\inlinesprite{0.02cm 2.02cm 4cm 2cm}}
\DeclareRobustCommand {\fountainsprite} {\inlinesprite{1cm 2cm 3cm 2cm}}
\DeclareRobustCommand {\wallsprite}     {\inlinesprite{2cm 2cm 2cm 2cm}}
\DeclareRobustCommand {\cratesprite}    {\inlinesprite{3cm 2cm 1cm 2cm}}
\DeclareRobustCommand {\predsprite}     {\inlinesprite{4cm 2cm 0cm 2cm}}
\DeclareRobustCommand {\spawnsprite}    {\inlinesprite{1cm 1cm 3cm 3cm}}
\DeclareRobustCommand {\exitsprite}     {\inlinesprite{2cm 1cm 2cm 3cm}}

\section{The SafeLife Environment} \label{safelife-env}

% \begin{itemize}
%     \item \textcolor{blue}{Basic Rules}
%     \item \textcolor{blue}{Three tasks}
%     \item \textcolor{blue}{Static vs Dynamic Environment}
% \end{itemize}


The SafeLife \citep{Wainwright2020} suite creates complex environments of systems of cellular automata based on a set of rules from Conway's Game of Life \citep{gardner1970fantastic} that govern the interactions between, and the state (alive or dead), of different cells:
\begin{itemize}
    \item any dead cell with exactly three living neighbors becomes alive;
    \item any live cell with less than two or more than three neighbors dies (as if by under- or overpopulation); and
    \item every other cell retains its prior state.
\end{itemize}
In addition to the basic rules, SafeLife enables the creation of complex, procedurally generated environments through special cells, such as spawner that can create new cells, and dynamically generated patterns. The agent can generally perform three tasks: \emph{navigation}, \emph{prune} and \emph{append} which are illustrated in Figure \ref{fig:simple-spawner} taken from \citep{Wainwright2020}.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.6in]{images/spawner.png}
    \caption{A simple level of the \emph{SafeLife} environment containing an agent~\mbox{(\agentsprite)}, a spawner~\mbox{(\spawnsprite)}, crates~\mbox{(\cratesprite)}, and dots of life. The agent's goal is to remove unwanted red dots (\emph{prune-task}) and to create new patterns of life in the blue squares (\emph{append-task}). Once the agent has satisfactorily completed its goals it can leave via the level exit~\mbox{(\exitsprite)}.
    Note that all level boundaries wrap; they have toroidal topology.}
    \label{fig:simple-spawner}
\end{figure}
The flexibility of SafeLife enables the creation of still environments, where the automata patterns do not change over time without agent interference, and dynamic environments, where the automata patterns do change over time without agent interference. The dynamic environments create an additional layer of difficulty, as the agent now needs to learn to distinguish natural variation and stochasticity in the environment from changes caused by its own actions. SafeLife has different information channels relaying rewards and side effects. The current side effect metric, as described in \citep{Wainwright2020} measures the change in a green automata from the starting state of the environment compared to the final state of the environment when the episode finishes. This metric can capture side effects relatively well for still environments, but is incomplete for dynamic environments where the automata pattern has a natural variation over time that is independent of the agent's actions.
\subsection{SafeLife Side Effect Metric}

The Safelife suite calculates the overall side effects at the end of the episode by taking a time-average of the state of the environment for a series of steps after the episode ends. This process is meant to ensure that the dynamics of the environment stabilize after the end of the agent ends the episode. In addition to the overall side effect at the end of the episode, SafeLife also has the option of producing an impact penalty for the agent during training. In the original SafeLife paper, \citep{Wainwright2020} uses that impact penalty to change the agent's reward function, whereas we are using the impact penalty as the side effect information channel in our co-training framework. The results reported in Section \ref{results} report the post episode side effect metric.
